Toward unsupervised, multi-object discovery in large-scale image collections

This paper addresses the problem of discovering the objects present in a collection of images without any supervision. We build on the optimization approach of Vo et al. (CVPR'19) with several key novelties: (1) We propose a novel saliency-based region proposal algorithm that achieves significantly higher overlap with ground-truth objects than other competitive methods. This procedure leverages off-the-shelf CNN features trained on classification tasks without any bounding box information, but is otherwise unsupervised. (2) We exploit the inherent hierarchical structure of proposals as an effective regularizer for the approach to object discovery of Vo et al., boosting its performance to significantly improve over the state of the art on several standard benchmarks. (3) We adopt a two-stage strategy to select promising proposals using small random sets of images before using the whole image collection to discover the objects it depicts, allowing us to tackle, for the first time (to the best of our knowledge), the discovery of multiple objects in each one of the pictures making up datasets with up to 20,000 images, an over five-fold increase compared to existing methods, and a first step toward true large-scale unsupervised image interpretation.

==> multiple_object_discovery.tex <==
\begin{table*}[htb]
    \centering
    \setlength{\tabcolsep}{1em}
    \begin{tabular}{cccccc}
        \toprule
        Method  & Features & OD & VOC\_6x2 & VOC\_all & VOC12 \\ 
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%
        Vo {\em et al.} RP & WHO &  &  & 40.7 $\pm$ 0.1 & - \\
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%
        Wei {\em et al.}~\cite{Wei2017ddt} & VGG16 & 71.8 & 46.9 & 37.1 & 39.5 \\
        Wei {\em et al.}~\cite{Wei2019ddtplus} & VGG16 & 76.5 & 48.9 & 38.3 & 40.4 \\
        Ours (OSD) & VGG16 & 77.6 $\pm$ 0.2 & 58.6 $\pm$ 0.1 & 45.9 $\pm$ 0.1 & 48.1 $\pm$ 0.0 \\
        Ours (rOSD) & VGG16 & \textbf{78.3 $\pm$ 0.1} & \textbf{58.9 $\pm$ 0.2} & \textbf{48.5 $\pm$ 0.1} & \textbf{50.7 $\pm$ 0.1} \\
        \midrule
        Wei {\em et al.}~\cite{Wei2017ddt} & VGG19 & 73.8 & 50.3 & 41.5 & 43.8 \\
        Wei {\em et al.}~\cite{Wei2019ddtplus} & VGG19 & 75.0 & 51.4 & 43.3 & 45.5 \\
        Ours (OSD) & VGG19 & 78.7 $\pm$ 0.0 & 59.6 $\pm$ 0.0 & 46.8 $\pm$ 0.1 & 47.9 $\pm$ 0.0 \\
        Ours (rOSD) & VGG19 & \textbf{77.8 $\pm$ 0.0} & \textbf{59.5 $\pm$ 0.2} & \textbf{49.4 $\pm$ 0.1} & \textbf{51.5 $\pm$ 0.1} \\
        \bottomrule
    \end{tabular}
    \caption{\small Multiple object discovery performance (\textit{detection rate}) in the separate setting on the datasets with our proposals compared to other works.}
    \label{table:multiple_separate}
\end{table*}

\begin{table*}[htb]
    \centering
    \setlength{\tabcolsep}{1em}
    \begin{tabular}{cccccc}
        \toprule
        Method  & Features & OD & VOC\_6x2 & VOC\_all & VOC12 \\ 
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%
        Vo {\em et al.} RP & WHO &  &  & 30.7 $\pm$ 0.1 & - \\
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%
        Wei {\em et al.}~\cite{Wei2017ddt} & VGG16 & 64.9 & 37.8 & 24.3 & 27.0 \\
        Wei {\em et al.}~\cite{Wei2019ddtplus} & VGG16 & 68.3 & 40.7 & 25.8 & 28.2 \\
        Ours (OSD) & VGG16 & 76.3 $\pm$ 0.0 & 53.6 $\pm$ 0.1 & 34.9 $\pm$ 0.1 & 37.6 $\pm$ 0.0 \\
        Ours (rOSD) & VGG16 & \textbf{77.3 $\pm$ 0.1} & \textbf{53.0 $\pm$ 0.2} & \textbf{37.2 $\pm$ 0.1} & \textbf{40.8 $\pm$ 0.1} \\
        \midrule
        Wei {\em et al.}~\cite{Wei2017ddt} & VGG19 & 62.5 & 36.7 & 26.4 & 28.6 \\
        Wei {\em et al.}~\cite{Wei2019ddtplus} & VGG19 & 63.1 & 38.0 & 28.1 & 30.3 \\
        Ours (OSD) & VGG19 & 78.2 $\pm$ 0.0 & 53.8 $\pm$ 0.1 & 34.8 $\pm$ 0.0 & 36.9 $\pm$ 0.0 \\
        Ours (rOSD) & VGG19 & 76.9 $\pm$ 0.0 & \textbf{53.5 $\pm$ 0.2} & \textbf{37.6 $\pm$ 0.1} & \textbf{40.4 $\pm$ 0.1} \\
        \bottomrule
    \end{tabular}
    \caption{\small Multiple object discovery performance (\textit{detection rate}) in the mixed setting on the datasets with our proposals compared to other works.}
    \label{table:multiple_mixed}
\end{table*}

